YOLO-RD: Introducing Relevant and Compact Explicit Knowledge to YOLO by Retriever-Dictionary

Identifying and localizing objects within images is a fundamental challenge, and numerous efforts have been made to enhance model accuracy by experimenting with diverse architectures and refining training strategies. Nevertheless, a prevalent limitation in existing models is overemphasizing the current input while ignoring the information from the entire dataset. We introduce an innovative Retriever-Dictionary (RD) module to address this issue. This architecture enables YOLO-based models to efficiently retrieve features from a Dictionary that contains the insight of the dataset, which is built by the knowledge from Visual Models (VM), Large Language Models (LLM), or Visual Language Models (VLM). The flexible RD enables the model to incorporate such explicit knowledge that enhances the ability to benefit multiple tasks, specifically, segmentation, detection, and classification, from pixel to image level. The experiments show that using the RD significantly improves model performance, achieving more than a 3\% increase in mean Average Precision for object detection with less than a 1% increase in model parameters. Beyond 1-stage object detection models, the RD module improves the effectiveness of 2-stage models and DETR-based architectures, such as Faster R-CNN and Deformable DETR. Code is released at https://github.com/henrytsui000/YOLO.

==> src/table/learning-curve.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{src/Visualize/AP95.pdf}
    \caption{Learning curve of Model vs RD-Model, the model with RD coverage speed is faster.}
    \label{fig: LR-curve}
\end{figure}


==> src/table/main_table.tex <==
\begin{table}[t]
\centering
\caption{Performance comparison of different models on the COCO 2017 validation set.}
\label{tab:model_comparison}
\begin{tabular}{lc|cccccc@{}}
\toprule
BackBone  & Initializer & Params & Atoms & Feature & $\text{mAP}^{val}_{.5}$ & $\text{mAP}^{val}_{.5:.95}$ \\ 
\midrule
YOLOv7      & Default   & 37.6M   & -       & -                        & 49.51\%      & 68.65\%     \\
YOLOv7      & YOLOv7    & 41.8M   & 4096    & $\mathbb{R}^{1024}$      & 49.95\%       & 68.94\%     \\
YOLOv7      & GPT       & 46.1M   & 4096    & $\mathbb{R}^{1024}$      & 49.86\%       & 69.24\%    \\
\midrule
YOLOv7      & Default   & 37.6M   & -       & -                        & 49.51\%       & 68.65\%  \\
YOLOv7      & YOLOv7    & 41.8M   & 4096    & $\mathbb{R}^{512}$       & 49.86\%       & 69.17\%     \\
YOLOv7      & CLIP(crop)& 41.8M   & 4096    & $\mathbb{R}^{512}$       & 50.15\%       & 69.61\%     \\
YOLOv7      & KD        & 38.1M   & 512     & $\mathbb{R}^{512}$       & 50.27\%       & 69.51\%        \\ 
YOLOv7      & mix\{GPT, CLIP\}& 41.8M & 4096& $\mathbb{R}^{512}$       & 49.88\%       & 69.29\%     \\
YOLOv7      & CLIP(orig)& 41.8M   & 4096    & $\mathbb{R}^{512}$       & 50.04\%       & 69.41\%     \\
YOLOv7      & CLIP(cvx) & 38.6M   & 1024    & $\mathbb{R}^{512}$       & 49.58\%       & 68.92\%     \\
YOLOv7      & Random    & 41.8M   & 4096    & $\mathbb{R}^{512}$       & 49.52\%       & 69.06\%        \\ 
YOLOv7      & VAE       & 41.8M   & 4096    & $\mathbb{R}^{512}$       & [CAL]\%       & [CAL]\%        \\ 
YOLOv7      & GPT2       & 41.8M   & 4096    & $\mathbb{R}^{512}$       & [CAL]\%       & [CAL]\%        \\ 
\midrule
YOLOv7-X      & Default    & 41.8M  & [TBD]   & [TBD]      & [EXP] & [EXP]        \\ 
YOLOv7-X      & YOLOv7     & 41.8M  & [TBD]   & [TBD]      & [EXP] & [EXP]        \\ 
YOLOv7-X      & CLIP       & 41.8M  & [TBD]   & [TBD]      & [EXP] & [EXP]        \\ 
\midrule
YOLOv7-E6      & Random    & 41.8M  & [TBD]   & [TBD]      & [EXP] & [EXP]        \\ 
YOLOv7-E6      & Random    & 41.8M  & [TBD]   & [TBD]      & [EXP] & [EXP]        \\ 
YOLOv7-E6      & Random    & 41.8M  & [TBD]   & [TBD]      & [EXP] & [EXP]        \\ 
\midrule
\midrule
GOLD-YOLO   & Default   & [CAL]  & -    & -      & [EXP]       & [EXP]     \\
GOLD-YOLO   & CLIP      & [CAL]  & [CAL]    & $\mathbb{R}^{1024}$       & [EXP]       & [EXP]     \\
GOLD-YOLO   & GPT      & [CAL]  & [CAL]    & $\mathbb{R}^{1024}$       & [EXP]       & [EXP]     \\
\midrule
\midrule
YOLOv9      & Default   & [CAL]  & -    & -      & 52.64\%      & 69.56\%     \\
YOLOv9      & CLIP      & [CAL]  & [CAL]    & $\mathbb{R}^{1024}$       & 53.23\%       & 70.28\%     \\
YOLOv9      & GPT       & [CAL]  & [CAL]    & $\mathbb{R}^{1024}$       & [EXP]       & [EXP]     \\
YOLOv9      & Default   & [CAL]  & [CAL]    & $\mathbb{R}^{1024}$       & [EXP]       & [EXP]     \\
\midrule
\midrule
Faster-RCNN      & Default   & [CAL]  & -    & -      & 52.64\%      & 69.56\%     \\
Faster-RCNN      & Vision-Model      & [CAL]  & [CAL]    & $\mathbb{R}^{1024}$       & 53.23\%       & 70.28\%     \\
Faster-RCNN      & VLM      & [CAL]  & [CAL]    & $\mathbb{R}^{1024}$       & 53.23\%       & 70.28\%     \\
Faster-RCNN      & LLM       & [CAL]  & [CAL]    & $\mathbb{R}^{1024}$       & [EXP]       & [EXP]     \\
\midrule
\midrule
DeTr      & Default   & [CAL]  & -    & -      & 52.64\%      & 69.56\%     \\
DeTr      & CLIP      & [CAL]  & [CAL]    & $\mathbb{R}^{1024}$       & 53.23\%       & 70.28\%     \\
DeTr      & GPT       & [CAL]  & [CAL]    & $\mathbb{R}^{1024}$       & [EXP]       & [EXP]     \\
\midrule
\end{tabular}
\end{table}


